MinRank Gabidulin encryption scheme on matrix codes

The McEliece scheme is a generic frame which allows to use any error correcting code of which there exists an efficient decoding algorithm to design an encryption scheme by hiding the generator matrix code. Similarly, the Niederreiter frame is the dual version of the McEliece scheme, and achieves smaller ciphertexts. We propose a generalization of the McEliece frame and the Niederreiter frame to matrix codes and the MinRank problem, that we apply to Gabidulin matrix codes (Gabidulin rank codes considered as matrix codes). The masking we consider consists in starting from a rank code C, to consider a matrix version of C and to concatenate a certain number of rows and columns to the matrix codes version of the rank code C and then apply to an isometry for matric codes. The security of the schemes relies on the MinRank problem to decrypt a ciphertext, and the structural security of the scheme relies on a new problem EGMC-Indistinguishability problem that we introduce and that we study in detail. The main structural attack that we propose consists in trying to recover the masked linearity over the extension field which is lost during the masking process. Overall, starting from Gabidulin codes we obtain a very appealing tradeoff between the size of ciphertext and the size of the public key. For 128b of security we propose parameters ranging from ciphertext of size 65 B (and public keys of size 98 kB) to ciphertext of size 138B (and public key of size 41 kB). Our new approach permits to achieve better trade-off between ciphertexts and public key than the classical McEliece scheme. Our new approach permits to obtain an alternative scheme to the classic McEliece scheme, to obtain very small ciphertexts, with moreover smaller public keys than in the classic McEliece scheme. For 256 bits of security, we can obtain ciphertext as low as 119B, or public key as low as 87kB.

==> encryption_mce.tex <==
\section{Encryption scheme}

\ac{Suggestion, est-ce qu'on ne pourrait pas appeler noise map une
  application de $\Cmat \rightarrow \Fq^{m\times (n+\ell)}$ définie
  par $N : \Xv \mapsto (\Xv ~|~ N_0 (\Xv))$ où
  $N_0 : \Cmat rightarrow \Fq^{m\times \ell}$. C'est juste que la notation
  $\Cmat^N$ je ne suis pas super fan. Je préfère $N(\Cmat)$.
Bon... je ne me battrai pas non plus pour ça :-)}

\paragraph{Key generation}
\begin{itemize}
	\item Pick a random Gabidulin (vector) code $\mathcal G[n,k]$.
	\item Pick a random $\Fq$-basis  $\gamma$ of $\Fqm$.
	\item Pick a random noise map $N \rand \mathcal L(\Cmat,\Fq^{m\times \ell})$
	\item Define the noisy matrix code $\Cmat := \Psi_\gamma(\mathcal G)^N$.
	\item Pick a random matrix $\Qv \in \mathbf{GL}_{n+\ell}(\Fq)$.
	\item Define the code $\Cmat' = \Cmat\Qv$.
	\item Let $\mathcal B = (\Mv_1,...,\Mv_{km})$ be a basis of $\Cmat'$
	\item Return \[
	\mathbf{pk} = \mathcal B \,;\, \mathbf{sk} = (\mathcal G, \gamma, \Qv)
	\]
\end{itemize}

\ac{En fait, est-ce qu'on prend un Gabidulin de longueur $n = m$?
  Parce qu'un Gabidulin est entièrement décrit par sa dimension et sa
  ``suite d'évaluations''. la suite d'évaluation peut être prise comme
  $\gamma$ ou les $n$ premiers termes de $\gamma$ si $n < m$. Ça ne
  change rien au niveau sécurité. La matrice $\Qv$ nettoie le choix de
  la ``séquence d'évaluation''.
  Bref, la clé secrète est $(k, n, \gamma, \Qv).$
}


\paragraph{Encryption}
~\\
Input: $\mathbf{pk} = (\Mv_1,...,\Mv_{km})$, $\mu \in \Fq^{km}$
\begin{itemize}
	\item Pick a random error matrix $\Ev \in \Fq^{m\times (n+\ell)}$ of rank $r$.
	\item Compute
	\[ \Yv := \sum_{i = 1}^{km} \mu_i \Mv_i + \Ev \]
	\item Return $\Yv$.
\end{itemize}

\paragraph{Decryption}
~\\
Input: $\mathbf{sk} = (\mathcal G, \gamma, \Qv)$, $\Yv \in \Fq^{m\times n}$
\begin{itemize}
	\item Compute $\yv$ be the first $n$ coordinates of the $(n+\ell)$-sized vector $\Psi_\gamma^{-1}(\Yv\Qv^{-1})$.
	\item Apply the decoding algorithm of $\mathcal G$ on the word $\yv$; it returns an error vector $\ev \in \Fqm^n$.
	\item Compute $\Ev' = \Psi_\gamma(\ev)$.
	\item Solve the linear system
	\[ \Yv - (\Ev'|\Nv)\Qv := \sum_{i = 1}^{km} \mu_i \Mv_i \] 
	whose $(k+\ell)m$ unknowns in $\Fq$ are the $\mu_i$ and the remaining part of the error $\Nv$ of size $m\times\ell$.
	\item Return the solution $\hat\mu$ of the above system.
\end{itemize}

\begin{proposition}[Decryption correctness]
When $r \le \frac{n-k}{2}$ and $k+\ell \le n$, the decryption algorithm outputs the correct message $\mu$.
\end{proposition}

\begin{proof}
	TODO. (Should be easy)
\end{proof}

==> encryption_nied.tex <==
\section{Encryption scheme}

We propose in this section an encryption scheme inspired by the Niederreiter cryptosystem: we mask by a secret operation (multiplication by a matrix $\Qv$ given in the secret key) the parity check matrix of a code for which we know a decoding algorithm. We use here a noisy Gabidulin code. However, rather than consider a vector code, we turn it into a matrix code, that we denote by $\Cmat$. It is then necessary to adapt the Syndrome Decoding approach to matrix codes, in the same way as what is presented in Subsection \ref{sec_MR}. The resulting scheme can be found in Figure \ref{enc_scheme}.

\begin{figure}[ht]
    \pcb[codesize=\scriptsize, minlineheight=0.75\baselineskip, mode=text, width=0.98\textwidth] { 
    $\KeyGen (1^\lambda)$: \\
    \pcind - Sample uniformly at random a basis $\gamma\getsr\mathcal{B}(\Fqm)$.\\
    \pcind - Construct the Gabidulin vector code $\mathcal G[m,k]_{q^m}$ whose evaluation points are the elements of $\gamma$.\\
    \pcind - Sample uniformly at random a noise map $N \getsr \mathcal L(\mathcal G,\Fq^{k\times \ell})$.\\
    \pcind - Define the noisy matrix code $\Cmat := \Psi_\gamma(\mathcal G)^N$.\\
    \pcind - Let $n=m+\ell$. Sample uniformly at random a matrix $\Qv \in \mathbf{GL}_n(\Fq)$.\\
    \pcind - Define the code $\Cmat' = \Cmat\Qv$. Let $\bar{\Hv}\in\Fq^{(n-k)m\times nm}$ a control matrix of $\Cmat'$.\\
    \pcind - Return $	\mathbf{pk} = \bar{\Hv} \,;\, \mathbf{sk} = (\gamma, \Qv)$\\[\baselineskip]
  %
  $\Encrypt (\pk,\mu)$: \\
  	\pcind \textit{Input:} $\pk=\bar{\Hv}$, a message $\mu \in \Fq^{nm}$ such that $\rank \Fold(\mu)\leq r$.\\
  	\pcind - For every integer $i$ from 1 to $nm$, let $\hv_i$ the i-th column of $\bar{\Hv}$. \\
	\pcind - Return $\cv = \sum_{i = 1}^{nm} \mu_i \hv_i^t$.\\[\baselineskip]
	%
	$\Decrypt (\sk,\cv)$:\\
	\pcind \textit{Input:} $\mathbf{sk} = (\gamma, \Qv)$, $\cv\in\Fqm^{(n-k)m}$.\\
	\pcind - Find any $\bar{\yv}\in\Fq^{nm}$ such that $\cv =\sum_{i=1}^{nm}\bar{y}_i \hv_i^t$.\\
	\pcind - Let $\Yv=\Fold(\bar{y})$. Compute $\yv= \Psi_\gamma^{-1}(\Yv)$.\\
	\pcind - Let $\yv=\mv\Gv+\ev$, with $\rank (\ev) \leq r$. Apply the decoding algorithm of $\mathcal G$ on the word constituted of the $n$ first coordinates.\\
	\pcind - Let $\Ev= \Psi_\gamma(\ev)$. Then $\Ev=(\Ev'|\Nv)\in\Fq^{m\times n}$ is a matrix whose the $m^2$ coefficients of $\Ev'$ are known, and $\Nv$ is the remaining part of the error.\\
	\pcind - $\bar{\ev}=\Unfold (\Ev)$.\\
	\pcind - Solve the linear system $\cv = \sum_{i=1}^{nm}\bar{e}_i \hv_i^t$ to find the values of $\Nv$.\\
	\pcind - Return $\hat\mu=\Unfold(\Ev\Qv^{-1})$.
}
\vspace{-\baselineskip}
\captionof{figure}{\footnotesize{Encryption scheme}}
\label{enc_scheme}
\end{figure}

\textbf{Comments.} The noisy Gabidulin $[n,k]_{q^m}$ isn't decodable on all its coordinates: the classical decoding algorithms for Gabidulin codes allow to decode only the $m$ first coordinates, but the random noise map avoid to decode the others. However, these $\ell$ coordinates can be recovered by solving a linear system of equations. On the other hand, using a matrix code, less structured than a vector code, increases the complexity of the attacks.

\begin{proposition}[Decryption correctness]
When $r \le \frac{m-k}{2}$ and $\ell\le n-k$, the decryption algorithm outputs the correct message $\mu$.
\end{proposition}

\begin{proof}
Let $\bar{\Gv}\in\Fq^{km\times nm}$ a generator matrix of the associated unfolded $\Cmat'$ vector code, and $\bar{\Hv}\in\Fq^{(n-k)m\times nm}$ a parity check matrix. Let $\bar{\yv}\in\Fq^{nm}$ such that $\Cv =\sum_{i=1}^{nm}\bar{y}_i\Mv_i$. Then: \begin{align*}
\Unfold (\Cv) &= \sum_{i=1}^{nm}\bar{y}_i\Unfold(\Mv_i)\\
&= \bar{\yv}\bar{\Hv}^t = \bar{\ev}\bar{\Hv}^t
\end{align*} where $\bar{\ev}=\Unfold ({\Psi_\gamma (\ev)})$.

The $m^2$ first values of $\bar{\ev}$ can be retrieved by decoding a word of the noisy Gabidulin code $\Psi_\gamma^{-1}(\Cmat')$. The rank of the error must not exceed the decoding capacity, i.e. $r \le \frac{m-k}{2}$.

The $\ell m$ last values can be retrieved by solving a linear system of $(n-k)m$ equations, which is possible if $\ell\le n-k$. Multiplying by $\Qv^{-1}$ allows to retrieve the original message $\mu$.
\end{proof}

==> quasirandom_codes.tex <==
\subsection{Quasi-random codes}

Here we define a new family of efficiently decodable codes. Close to random codes and therefore very unstructured, we take advantage of their small size to deduce an immediate decoding algorithm.

Let $\Gv\in\Fqm^{k\times n}$ the generator matrix of a $[n,k]_{q^m}$ linear code $\C$, $\yv=\xv\Gv+\ev$ a noisy codeword, with unknown $\xv\in\Fqm^k$ and $\ev\in\Fqm^n$ an error of weight $\wrank{\ev}=r$.\\
We try to decode this codeword by retrieving the support of the error. Let $A=\sum_0^{r-1} a_iX^{[j]}+X^{[r]}$ the q-polynomial of q-degree $r$ that erases the support of $\ev$. For a vector $\vv=(v_1,...,v_n)$, we abusively denote by $A(\vv)$ the vector $(A(v_1),...,A(v_n))$. This calculus follows:

\begin{align*}
A(\yv) &= A(\xv\Gv) + A(\ev) &\text{by linearity of }A\\
&= A(\xv\Gv) &\\
&= \sum_{i=1}^k A(x_i\gv_i) &\text{with }\gv_i\text{ as the rows of }\Gv\\
&= \sum_{i=1}^k\sum_{j=1}^r a_jx_i^{[j]}\gv_i^{[j]}+x_i^{[r]}\gv_i^{[r]}&(1)\\
\end{align*}

We can deduce from the vectorial equality (1) a linear system of $n$ equations by considering as unkowns the $r(k+1)$ following values: $a_jx_i^{[j]}$ and $x_i^{[r]}$. If the parameters verify $k(r+1)\leq n$, and the coefficients of $\Gv$ must be such that the system has a solution, then one can straightfowardly decode any error of rank $r$ by solving this system. This property on the code is denoted as Property 1, that we formally define below:

\textbf{Property 1.} $\C$ is a vector code $[n,k,r]$ on $\Fqm$ such that $r(k+1)\leq n$ and the system of equations of unkowns $a_jx_i^{[j]}$ and $x_i^{[r]}$ deduced from (1) can be solved.

\begin{definition}[Quasi-random code]
Let integers $m,n,k,r\in\mathbb{N}$, $q$ a prime or a power of prime. A Quasi-random code $\Q(n,k,r)$ over $\Fqm$ is a $[n,k,r]$ code which verifies the Property 1.
\end{definition}

\textit{Remark.} By sampling a $[n,k,r]$ code uniformly at random such that $k(r+1)\leq n$, we obtain a Quasi-random code with a very high probability.

\begin{proposition}
A $\Q(n,k,r)$ code disposes of a decoding algorithm capable of decoding errors of rank up to $r$, and needs at most $O(r^3(k+1)^3)$ multiplications in $\Fqm$.
\end{proposition}

\begin{proof}
A linear system of $N$ equations can be solved with Gaussian elimination, which needs at most $O(N^3)$ multiplications in the base field. \qed
\end{proof}

==> signature.tex <==
\section{Signature scheme}
For the signature, we take $m = n$.
In that setting, the rank Gilbert-Varshamov bound verifies $d_{RGV} \approx n(1-\sqrt{k/n})$.

\paragraph{Key generation}
\begin{itemize}
	\item Pick a random Gabidulin (vector) code $\mathcal G[n,k]$.
	\item Pick a random $\Fq$-basis of $\Fqm$ $\gamma$.
	\item Pick a random matrix code $\mathcal R_{mat}$ of size $m\times (n+\ell)$ and dimension $m\ell$.
	\item Define the matrix code $\Cmat := (\Psi_\gamma(\mathcal G) \,|\, \mathbf{0}) \oplus \mathcal R_{mat}$ (the zero block appended to $\Psi_\gamma(\mathcal G)$ is of size $m \times \ell$).
	\item Pick a random matrix $\Qv \in \mathbf{GL}_{n+\ell}(\Fq)$.
	\item Define the code $\Cmat' = \Cmat\Qv$.
	\item Let $\mathcal B = (\Mv_1,...,\Mv_{(k+\ell)m})$ be a basis of $\Cmat'$
	\item Return \[
	\mathbf{pk} = \mathcal B \,;\, \mathbf{sk} = (\mathcal G, \mathcal R_{mat}, \gamma, \Qv)
	\]
  \end{itemize}

  \ac{Même commentaire, pas besoin de mettre $\mathcal G$ dans la clé
    secrète.}

\paragraph{Signature}
~\\
Input: $\mathbf{sk} = (\mathcal G, \gamma, \Qv)$, $\mu \in \{0,1\}^{*}$
\begin{itemize}
	\item Let $i = 0$.
	\item Compute $\Yv = \mathcal H(\mu || i)$. $\mathcal H$ is a hash function that outputs elements in $\Fq^{m\times (n+\ell)}$.
	\item Let $\Yv' := \Yv\Qv^{-1}$.
	\item Let $T \rand \gr(\Fqm, \ell)$ a random subspace of dimension $\ell$.
	\item Let $(e_1, ..., e_\ell)$ be a random basis of $T$.
	\item Let $\Ev_2 = \Psi_\gamma(e_1, ..., e_\ell)$ be an
      $m \times \ell$ matrix.
	\item Find $\Rv \in \Rmat$ such that $\Yv' - \Rv$ is of the form $(\Yv'' \,|\, \Ev_2)$.
	\item If such an $\Rv$ can't be found, increase $i$ by one and return to step 2.
	\item Compute $\yv'' := \Psi_\gamma^{-1}(\Yv'')$.
	\item Apply the decoding algorithm of $\mathcal G$ on the word $\yv''$ with support erasure $T$.
	\item If it doesn't work, increase $i$ by one and return to step 2.
	\item If it works, it returns an error vector $\ev \in \Fqm^n$ such that:
	\begin{itemize}
		\item $(\yv'' - \ev) \in \mathcal G$
		\item $T \subset \Supp(\ev)$ 
		\item $\dim(\Supp(\ev)) \le(n-k+\ell)/2$
	\end{itemize}
	\item Compute $\Ev = (\Psi_\gamma(\ev) \,|\, \Ev_2)\Qv$.
	\item Return $\mathbf{\Sigma} = (\Ev, i)$.
\end{itemize}

\paragraph{Verification}
~\\
Input: $\mathbf{pk} = (\Mv_1,...,\Mv_{km})$, $\mathbf{\Sigma} = (\Ev, i) \in \Fq^{m\times n} \times \mathbb N$, $\mu \in \{0,1\}^{*}$
\begin{itemize}
	\item Verify that $\Ev$ is of rank $\le (n-k+\ell)/2$.
	\item Compute $\Yv = \mathcal H(\mu || i)$.
	\item Verify that $\Yv - \Ev$ belongs to the code defined by the public key $\mathbf{pk}$.
\end{itemize}

\begin{proposition}[Verification correctness]
	For any message $\mu$, if $\mathbf{\Sigma}$ = \textnormal{Sign(}$\sk, \mu$\textnormal{)}, then \textnormal{Verif(}$\pk, \mathbf{\Sigma}, \mu$\textnormal{)} outputs \textnormal{True}.
\end{proposition}

\begin{proof}
Let $\mathbf{\Sigma} = (\Ev, i)$ and $\Yv = \mathcal H(\mu || i)$. We keep the same notation as above. It is readily seen, thanks to the decoding algorithm with support erasures, that the column space of $\Ev_2$ is included in the column space of $\Psi_\gamma(\ev)$. Therefore, $\Ev$ is of rank $\le (n-k+\ell)/2$.

It remains to prove that $\Yv-\Ev \in \Cmat'$. We have
\begin{align*}
\Yv-\Ev &= [\Yv' - (\Psi_\gamma(\ev) \,|\, \Ev_2)]\Qv \\
&= [\Rv + (\Yv'' \,|\, \Ev_2) - (\Psi_\gamma(\ev) \,|\, \Ev_2)]\Qv\\
&= [\Rv + (\Psi_\gamma(\yv'' - \ev)\,|\, \mathbf{0})]\Qv
\end{align*}
Since $(\yv'' - \ev) \in \mathcal G$ and  $\Rv \in \Rmat$, we have that $\Rv + (\Psi_\gamma(\yv'' - \ev)\,|\, \mathbf{0}) \in \Cmat$. We thus immediately deduce $\Yv-\Ev \in \Cmat'$. \qed
\end{proof}

\begin{proposition}
The density of signable matrices (i.e. the proportion of matrices $\Yv$ for which an error $\Ev$ can be found through the signature algorithm described above) is approximately
\[ q^{-(\frac{n-k-\ell}{2})^2}\]
\end{proposition}

\begin{proof}
	TODO.
\end{proof}
